Composable constraints

We introduce a notion of compatibility between constraint encoding and compositional structure. Phrased in the language of category theory, it is given by a "composable constraint encoding". We show that every composable constraint encoding can be used to construct an equivalent notion of a constrained category in which morphisms are supplemented with the constraints they satisfy. We further describe how to express the compatibility of constraints with additional categorical structures of their targets, such as parallel composition, compactness, and time-symmetry. We present a variety of concrete examples. Some are familiar in the study of quantum protocols and quantum foundations, such as signalling and sectorial constraints; others arise by construction from basic categorical notions. We use the language developed to discuss the notion of intersectability of constraints and the simplifications it allows for when present, and to show that any time-symmetric theory of relational constraints admits a faithful notion of intersection.

==> figures/spare2.tex <==
\color{red} More Matt chatting to matt garbage
\subsubsection{Possible Solution}
We introduce a partial order on $\cat{Dot[V]}$ which captures structural deduction. We can then even go further and define practical isomatry and practical causality in terms of this partial order!



%What is the meaning of a single diagram or term of morphisms when written down for a user? The term $f \circ g$ means the morphism $f$ composed with the morphism $g$, so far so obvious. The user is imagined to keep track of who $f$ and $g$ are seperately and to now in their head carry the concept of having composed $f$ with $g$. Note that just because some equation $h  =  f \circ g$ holds in a category $\cat{V}$ does not mean that the user knows that yet, as such the term $f \circ g$ does not mean $h$ to a user, even if it really is $h$. The equation $h = f \circ g$ is an (albeit simple) decomposition theorem, a piece of knowledge that the user may or may not be aware of. We labour this distinction because of the quite strange meaning of $(f,\tau)$. Here the user sees two morphisms \textbf{and} an equation, it is a state of knowledge. What then should be the meaning of $(f,\tau) \circ (g \circ \sigma)$? in particular, what does it mean to write down this diagram?


%A user can write down $f \circ g$ and a user can go further and use the assigment or formular for $\circ$ to compute $f \circ g$. When the latter is written on the page and shown to someone else it carries a different piece of data. Given the equations of the category $\cat{V}$ one would know that they were the same piece of data. 
\subsubsection{Possible Solution 2}
So what EXACTLY is the problem here? 
What is the purpose of a diagram of routing morphisms? Once written down it should represent
\begin{itemize}
    \item The global process that will occur
    \item The localised processes which make it up
    \item The conditions those processes obey in terms of where they distribute information
\end{itemize}
The first two ideas are essentially a decomposition theorem. The statement $h = f \circ g$ is an equation which represents a decomposition theorem. The statement $h = (f,\tau) \circ (g, \sigma)$ is a new decomposition theorem, it tells us that $h$ decomposes into some morphisms, and those morphisms satisfy some conditions. In the former example $f \circ g$ there is no statement on $f$ or $g$ so there is no way to say that one could equivalently written $f'$ where $f'$ is a looser condition than $f$. Here we have such a situation, we have a relation on morphisms that we want to use, to say that having the decomposition $(f,\tau)$ after $(g,\sigma)$ implies having some other decomposition. 

We have a composition rule but the composition rule doesn't really have the same meaning as the diagram to a user. When a user reads a term $(f,\tau) \circ (g,\sigma)$ they have more information than is in the term $(f \circ g, \tau \sigma)$. To capture this, and the fact that part of what our terms represent is the users knowledge, we define a new formal category of terms, which has on it a partial order. The user performs computations by moving through the partial order of the freely generated category. 
\begin{definition}[Freely Generated Category]
The category $\cat{f}(\cat{V})$ freely generated by $\cat{V}$ has as objects the objects of $\cat{V}$ and as morphisms in $\cat{f}(\cat{V})(A,B)$, finite lists of morphisms $[f_1 \dots f_n]$ such that the header $f_1 : A \rightarrow X$ and the tail $f_n: Z \rightarrow A$
\end{definition}
We start with $\cat{f}(\cat{Dot}(\cat{V}))$ and then we can define a new category identifying morphisms by structural equivalence. 
\begin{definition}
The category $\cat{S}(\cat{f}(\cat{Dot}(\cat{V})))$ has as objects the objects of $(\cat{f}(\cat{Dot}(\cat{V}))$ and as morphisms the morhpisms
\end{definition}
\subsubsection{Possible Solution 3}
We could simply hack the problem by defining a new relation starting with a relaxed version of implication. 
\begin{align*}
    (f,\tau) \bar{\geq} (f,\tau') \iff \textbf{ either } (f,\tau) \geq (f,\tau') \\
    \textbf{or } \textrm{there exists } (f_1,\sigma),(f_2,\lambda) (f_1,\sigma'),(f_2,\lambda') \textrm{ such that }  (f_1,\sigma) \geq (f_1,\sigma') \textrm{ and } (f_2,\lambda) \geq (f_2,\lambda') \textrm{ and } \\
    (f,\tau) = (f_1,\sigma) \circ (f_2,\lambda) \\
    (f,\tau) = (f_1,\sigma') \circ (f_2,\lambda')
\end{align*}
Looks nasty but pretty simple. The drawback is that now there are morphisms which we call equivlanet even though we would need to know how they composed to show they were equivalent. On the plus side however, it means the nasty counter example about a morphism which is not $CPM$ of some morphism dissapears. Here is the proof that that nasty counter example is now handled. 

\begin{lemma}[Coherent Specifics are Equivlanet to CPM'm maps now]
Take that state $\rho =$ which has a completely positive relation $\tau = $. Then this morphism is equivalent to a morphism of the form $\CPM[(\psi, \tau)]$.
\end{lemma}
\begin{proof}
Blah
\end{proof}


\color{black}


\subsubsection{Possible Solutions}
Accept that there are two types of calculations in the world now, 
\begin{itemize}
    \item Ones where we show that morphisms are equal to other morphisms 
    \item One where we show that statements of knowledge (Presented as Morphisms) imply other statements of knowledge (Presented as Morphisms)
\end{itemize}
The wierd feature of $(f,\tau) \circ (g,\sigma)$ is that it is a state of knowledge equal to (by definition) $(f \circ g, \tau \circ \sigma)$ even though us having written down the expression $(f,\tau) \circ (g,\sigma)$ requires more knowledge than writing down the statement $(f \circ g, \tau \circ \sigma)$. 

When a user writes down an expression, they could compute $\circ$ to make new morphisms with new conditions on them, or they could look at their expression, a state of knowledge about some morphisms an how they have been composed, and make some deductions from it (for example by making ).

If we want to perform calculations involving decoherences and trace outs. We can do the following to some expression $f_1 \circ \dots \circ f_n$. Our end goal is after partial tracing to find out what the new morphism is, and how it is routed. 
\begin{itemize}
    \item Plug the partial trace into the expression
    \item We have computed a new morphism and we have some not very useful information about how it is routed,
    \item We can perform a deduction on the expression to show that 
\end{itemize}
and then the interesting feature of this double setting where we compute morphisms and derive statements about them, is that the deductions don't necessarily commute with composition, so if we want to learn as much as possible about the routing behaviour of a global morphism we should always perform all the deductions we can before computing a composition. 

Now the thing is, in a category there is no meaning in an expression $f \circ g$ prior to computing the composition. As far as the category is concerned $f \circ g$ Is whatever we WILL compute it to be. However given a restricted set of allowed equations it could well be that there are things that we can show are equal to $f \circ g$ by for example replacing $f$ by some morphisms we know it to be equal to, but that we cannot prove are equal to the computed version of $f \circ g$. The takeaway is that even in the standard setting: Once we only allow some equations from a category to be used, equality derivable by those rules is not guaranteed (nor expected) to be compositional. We could even view composition itself as being an allowed or non allowed equation?

The long and short of all of this, is that it feels like to explain what the point is in dot diagrams, routed morphisms are etc, we need to be explicit about what a computation is etc. 

It feels like what we want to say is something about the free monoidal category generated by $\cat{Dot[V]}$. This is the category of expressions built from $\cat{Dot[V]}$. For instance there is a formal expression $f \circ g$ and in particular it is not equal to the $h \in \cat{Dot[V]}$ such that in $\dot[V]$ $h = f \circ g$. 

Given a formal expression $f_1 \circ \dots \circ f_n$ what can we do? This is the kind of thing that appears on someones piece of paper. Well one could use an equation from the category to compute $f_1 \circ f_2$ for example, or one could use the fact that $f_1 > f_1'$ to derive that


==> figures/sparenotes.tex <==
\section{Special commutative $\dagger$-Frobenius algebras}
Let me unashamedly plagiarise \cite{Coecke_2014}.

\begin{definition}
  A \textbf{Frobenius algebra} is an object $A$ in a monoidal category together
  with morphisms depicted as $\whitemult$, $\whiteunit$, $\whitecomult$
  and $\whitecounit$ on it satisfying the following diagrammatic equations.
%  \c% tikzfig{fa_axioms}
\end{definition}

Any Frobenius algebra defines a cap and a cup that satisfy the snake equation:
%\be \label{cap_cup} \tikzfig{cap_cup} \ee

Here we will restrict to dagger compact categories and to Frobenius algebras which play naturally with the dagger.

\begin{definition} In a dagger compact category \cat{V}, a $\dagger$\textbf{-Frobenius
algebra} is a Frobenius algebra that satisfies $\whitecomult = (\whitemult)^\dag$ and
$\whitecounit = (\whiteunit)^\dag$.
\end{definition}

Of particular interest are \textit{special commutative} $\dagger$-Frobenius algebras.

\begin{definition} A $\dagger$-Frobenius algebra is \textbf{commutative} if $\sigma_{A,A} \circ \whitecomult = \whitecomult$, where $\sigma$ is the swap morphism.
\end{definition}

\begin{definition} A $\dagger$-Frobenius algebra is \textbf{special} if $ \whitemult \circ \whitecomult = \tr{id}_A \, .$
\end{definition}

In \FHilb, "a special commutative $\dagger$-Frobenius algebra" is just a pretentious way of saying "a Hilbert space with a preferred basis", as the holy laws of category theory forbid the use of such a low-level notion as that of a basis\footnote{ahah additive structure go brrrrr}. The spider is the copying operation in that basis.

We will now present further theorems on some features of $\dagger$-Frobenius algebras. First, the Frobenius structure allows states to act on the space; this defines a specific kind of morphisms.

\begin{definition} If $A$ is a $\dagger$-Frobenius algebra in \cat{V}, a \textbf{diagonal morphism} on $A$ is a morphism from $A$ to itself in \cat{V} of the form
%\be \tikzfig{diagonal2} \quad = \quad \tikzfig{diagonal} \, .\ee
\end{definition}

Thus, there is a correspondence between states on $A$ and diagonal morphisms of $A$. This gives meaning to the following definitions, which assign to states some properties of their associated diagonal morphism.

\begin{definition} If $A$ is a $\dagger$-Frobenius algebra in \cat{V}, a state $\iota$ on $A$ is \textbf{invertible} if there is a state $\iota^{-1}$ on $A$ such that $\whitemult \circ ( \ket{\iota} \otimes \ket{\iota^{-1}}) = \whitemult \circ ( \ket{\iota^{-1}} \otimes \ket{\iota}) = \whiteunit$.
\end{definition}

\begin{definition} If $A$ is a $\dagger$-Frobenius algebra in \cat{V}, a state $\tau$ on $A$ is \textbf{idempotent} if $\whitemult \circ ( \ket{\tau} \otimes \ket{\tau}) = \ket{\tau})$.
\end{definition}

\begin{example}\label{IdempotFHilb}
Let $Z_A$ be a special commutative $\dagger$-Frobenius algebra in $\FHilb$, specified by an ONB $\{ \ket{a_i} \}$ of $Z_A$. Idempotents $\ket{\tau}$ on $Z_A$ are exactly the states of the form $\ket{\tau} = \sum_i \tau_i \ket{a_i}$, where the $\tau_i$ are in $\{ 0, 1 \}$.
\end{example}

Note that whenever we talk about invertible or idempotent states on a Frobenius algebra, we are referring to morphisms in \cat{V}, not to homomorphisms of Frobenius algebras.

There is a natural way of composing two $\dagger$-Frobenius algebras in parallel to get another one:

\begin{theorem} \label{TensorFrob} If $(A, \whitemult, \whiteunit)$ and $(B, \graymult, \grayunit)$ are two $\dagger$-Frobenius algebras in \cat{V}, then $(A \otimes B, (\whitemult \otimes \graymult) \circ (\tr{id}_A \otimes \sigma_{A,B} \otimes \tr{id}_B), \whiteunit \otimes \grayunit)$ is a $\dagger$-Frobenius algebra too. If $A$ and $B$ are both commutative (resp. special), then $A \otimes B$ is too. Tensor products of invertible (resp. idempotent) states are invertible (resp. idempotent).
\end{theorem}

\begin{proof} Well if you try it it works \end{proof}

Next, we define the notion of normalised partial trace of an idempotent. If we have two special commutative $\dagger$-Frobenius algebras $Z_A$ and $Z_B$, and an idempotent on $Z_A \otimes Z_B$, we want to obtain an idempotent on $A$ out of it. The idea is to do this by using equivalence classes under product with invertible states. Let us give a name to categories in which this is a well-defined operation, and show that \FHilb is one of them.

\begin{definition} \label{NormTrace} A $\dagger$ compact closed category \cat{V} \textbf{admits a normalised trace on idempotents}\footnote{The rigorous way to state it would be to say that it admits a normalised partial trace on idempotents on its special commutative $\dagger$-Frobenius algebras, but this is starting to be a bit long.} if it satisfies the following property: let $Z_A$ and $Z_B$ be two special commutative $\dagger$-Frobenius algebras in \cat{V}, and $\tau$ be an idempotent on $Z_A \otimes Z_B$. Then there exists a unique idempotent $\tilde{\tau}$ on $Z_A$ satisfying:

%\be \exists \iota \tr{, invertible, such that  } \quad \% tikzfig{NormTrace1} = \tikzfig{NormTrace2} \, .\ee

$\tilde{\tau}$ is called the \textit{normalised partial trace on} $Z_B$ of $\tau$, written $\tl{\tau} = \Tr_{Z_B}(\tau)$.

\end{definition}

\begin{theorem} $\FHilb$ admits normalised traces on idempotents.
\end{theorem}

\begin{proof}
In \FHilb, the Frobenius algebras on $Z_A$ and $Z_B$ are given by ONBs $\{ \ket{a_i} \}$ and $\{ \ket{b_j} \}$. Following example \ref{IdempotFHilb}, $\ket{\tau} = \sum_{ij} \tau_{ij} \ket{a_i} \otimes \ket{b_j}$, so $(\tr{id} \otimes \graycounit) \circ \ket{\tau} = \sum_i (\sum_j \tau_{ij}) \ket{a_i} $. As multiplication with an invertible state here means multiplying each coefficient in the decomposition by a non-zero number, it is clear that only one idempotent can be obtained from this by multiplying with an invertible state: namely, $\ket{\tl{\tau}} = \sum_i  \tl{\tau}_{i} \ket{a_i}$ where $ \tl{\tau}_{i}$ is equal to $0$ if $\sum_j \tau_{ij} = 0$, and $1$ otherwise.
\end{proof}

I have no idea whether such a theorem is true in all compact closed categories; this should be further looked into.

There is another property of partial traces of idempotents which we will need later.

\begin{definition}
In a $\dagger$-compact closed category $\cat{V}$, admitting normalised traces on idempotents, the normalised partial trace on $Z_B$ is \textbf{loosening} on a state $\tau$ on $Z_A \otimes Z_B$ if the product of $\Tr_{Z_B}(\tau) \otimes \grayunit_{Z_B}$ with $\tau$ is equal to $\tau$.
\end{definition}

\begin{theorem}
In \FHilb, all partial traces are loosening.
\end{theorem}

\begin{proof}
.
\end{proof}

Once again I have no idea whether this holds in general.

The existence of a normalised (not necessarily loosening) trace on idempotents allows to define a category of idempotents on Frobenius algebras.

\begin{definition}
Let \cat{V} be a dagger compact closed category admitting normalised traces on idempotents. The category \cat{FrobIdempot[V]} is the category in which:

\begin{itemize}
\item objects are special commutative $\dagger$-Frobenius algebras in \cat{V};
\item morphisms from $Z_A$ to $Z_B$ are idempotents on $Z_A \otimes Z_B$ in $\cat{V}$;
\item the identity on $Z_A$ is the cup on $Z_A$ defined in (\ref{cap_cup});\item composition (noted $\tl{\circ}$) of $\tau : Z_A \to Z_B$ and $\sigma : Z_B \to Z_C$ is given by
\be \sigma \tl{\circ} \tau = \Tr_{Z_B} \left( (\tr{id}_{Z_A} \otimes \graymult_{Z_B} \otimes \tr{id}_{Z_C}) \circ (\tau \otimes \sigma) \right) \, .\ee
\end{itemize}
\end{definition}
I will eventually write down the proof that this is a category, but in the meantime I leave it as an exercise to the reader as it's genuinely not a bad idea to try and work out how it behaves.

This category of Frobenius idempotents is endowed with all the structure we like:

\begin{theorem}
\cat{FrobIdempot[V]} is a $\dagger$-compact closed category in which:
\begin{itemize}
\item tensor product is given by the tensor product of Frobenius algebras described in Theorem \ref{TensorFrob};
\item the unit object is the Frobenius algebra naturally defined on the unit object $1$ of \cat{V};
\item the adjoint of $\tau: Z_A \to Z_B$ is given by $\sigma_{Z_A Z_B} \circ \tau$, where $\sigma_{Z_A Z_B}$ is the swap isomorphism in $\cat{V}$;
\item every object is self-dual;
\item the unit on $Z_A$ is given by the cup as defined in theorem $\ref{cap_cup}$.
\end{itemize}
\end{theorem}

For $\FHilb$, the category of Frobenius idempotents is another guise of an old friend.

\begin{theorem}
\cat{FrobIdempot[FHilb]} is equivalent to \FRel, the category of relations between finite sets.
\end{theorem}

\begin{proof}
(Sketch) The idea would be to use Theorem 5.64 in \cite{coecke_kissinger_2017} (I don't know where this theorem was proven in the literature) to prove that \cat{FrobIdempot[FHilb]} is equivalent to \cat{Mat(B)}, the category of matrices on the booleans, which is itself equivalent to \FRel. The theorem requires the existence of enrichment in sums; these can be defined in \cat{FrobIdempot[FHilb]} by using sums in \FHilb then renormalising as we did in Theorem \ref{NormTrace}. The other assumptions of the theorem are that each object has an ONB, and that there exist objects of every dimension: these are verified easily. Therefore \cat{FrobIdempot[FHilb]} is equivalent to the category of matrices over its scalars; the latter are clearly the booleans.
\end{proof}

\section{The category of dots}

Let us first define partitions using Frobenius algebras, through the use of module coactions.

\begin{definition} In a compact closed category \cat{V}, a \textbf{partition} of an object $A$ is given by a special commutative $\dagger$-Frobenius algebra $Z_A$ and a morphism $\whitemeas : A \to A \otimes Z_A$, called a module coaction, satisfying:

\begin{subequations}
\be \label{ModuleActionA} (\whitemeas \otimes \tr{id}_{Z_A}) \circ \whitemeas = ( \tr{id}_A  \otimes \whitecomult ) \circ \whitemeas \,  ; \ee
\be \label{ModuleActionB}  (\tr{id}_A \otimes \whitecounit) \circ \whitemeas = \tr{id}_A \, . \ee
\end{subequations}
\end{definition}

We can see that partitioning $A$ means equipping it with a preferred module structure over a special commutative $\dagger$-Frobenius algebra. %In \FHilb, for orthogonal partitions, one could think of the module coaction $\whitemeas$ as a degenerate measurement; but in the context in which we will use it, this would lead to confusion as there are no physical measurements involved - rather, its use will be to enforce correlations between \textit{potential} measurements. In addition, this is not a measurement going from the doubled theory to the single one - everything is happening at the single level here.

Another requirement singles out orthogonal partitions.

\begin{definition} A given partition is \textbf{orthogonal} if, noting $\whitecomeas := (\whitemeas)^\dagger$,
\be \label{OrthModule} \whitecomeas = (\tr{id}_A \otimes \whitecap_{Z_A}) \circ (\whitemeas \otimes \tr{id}_{Z_A}) \, . \ee
\end{definition}

The following can be useful:

\begin{theorem}
The module coaction $\whitemeas$ of an orthogonal partition is an isometry.
\end{theorem}
\begin{proof}

%\be \tikzfig{MeasAdj0} \overset{(\ref{OrthModule})}{=} \% tikzfig{MeasAdj1} \overset{(\ref{ModuleActionA})}{=} \% tikzfig{MeasAdj2} \overset{(\tr{specialness})}{=} \% tikzfig{MeasAdj3} \overset{(\ref{ModuleActionB})}{=} \% tikzfig{MeasAdj4} \, . \ee
\end{proof}

In \FHilb, specifying an orthogonal partition of $A$ corresponds to specifying a certain decomposition of it into orthogonal subspaces, $A = \oplus_{i=1}^n A^i$, where $n$ is the dimension of $Z_A$. We will use this and idempotents on special commutative $\dagger$-Frobenius algebras to build a category in which morphisms feature constraints as to which subspace in the domain can be mapped to which subspace in the codomain.

\begin{definition}
Let \cat{V} be a dagger compact closed category admitting partial traces on idempotents, and in which all partial traces are loosening. \cat{Dot[V]} is the category in which:

\begin{itemize}
\item objects are orthogonal partitions $(A, Z_A)$ in \cat{V};
\item morphisms from $(A, Z_A)$ to $(A, Z_B)$ are pairs $(f, \tau)$ where $f \in \cat{V}(A,B)$, $\tau \in \cat{FrobIdempot[V]}(Z_A, Z_B)$ and 
%\be \tikzfig{FrobIdempot} = \% tikzfig{FrobIdempot2} \, ; \ee
 $\tau$ is called a \textbf{routing morphism} of $f$;
\item composition is given by $(g, \sigma) \circ (f, \tau) = (g \circ f, \sigma \tl{\circ} \tau)$.
\end{itemize}
\end{definition}

The non-trivial thing to check in order to ensure that this is indeed a category is the following.

\begin{theorem}
Composing two morphisms in \cat{FrobIdempot[V]} yields a morphism in \cat{FrobIdempot[V]}.
\end{theorem}

\begin{proof}
The requirement that all partial traces should be loosening is central here.
\end{proof}

\begin{theorem}
From the structures of $\dagger$-compact closed categories on \cat{V} and \cat{FrobIdempot[V]}, one can endow \cat{Dot[V]} with the structure of a $\dagger$-compact closed category by defining all operations (tensor products, unit objects, adjoints, duals, units) pairwise.
\end{theorem}

\begin{proof}
Should be routine (?)
\end{proof}


\subsection{Structural Deductions (Warning - Could be Dead End)}
A routing map $(f,\tau)$ is a state of knowledge about how $f$ distributes information between subspaces. In this section we propose a suitable notion of equivalences between to states of knowledge $(f,\tau)$ and $(f,\tau')$. It is often the case that there are facts about particular morphisms, which are so self evident to the user, that it feels as if they should be built into the calculus given to the user. A motivating example is the $\cap$. It takes no effort to show that statement $``(\cap,\cap)"$.
\begin{equation}\label{cap}
    \tikzfigscale{1}{cap}
\end{equation}
However when using the calculus as it currently stands, the only method that we have for deriving new routing morphisms from old ones is composition, and this is not sufficient to even retain the knowledge of the self evident statement $(\cap,\cap)$. For example for any trace preserving map $f$ we have $(\cap,\cap) \circ (f,\tau)  = (\cap, \cap \circ \tau)$, where there is no garuntee at $\cap \circ \tau = \cap$. In fact as a counterexample let $\tau_{ij}^{kl} = 1$ for all $i,j,k,l$ then $(\cap \circ \tau)_{ij} = 1$ for all $i,j$ and so $(\cap \circ \tau) \neq \cap$.





A trivial solution is to allow for $(f,\tau)$ and $(f,\tau')$ to be equivalent whenever we can use $(f,\tau)$ to prove $(f,\tau')$ and vice-verse. But if we allow ourselves to use all equations in $\cat{V}$ to make such deductions, all $(f,\tau)$ and $(f,\tau')$ immediately become equivalent, the equivalence classes absorb any knowledge about the routing information! 

Our goal is then to agree on the allowed deductions we may use, the calculus should not treat as distinct those statements which are provable through the structure used to define the calculus. However the calculus should treat as distinct all of those statements which are true only due to the particular properties of $\cat{V}$. We argue that we should use the equations that we have already for free, and no more. By equations that we already have for free we mean that we wish to only use the structure - the equations that must be satisfied to even define $\cat{Dot}{\cat{V}}$. For us this means that we may use the equations which come for free from dagger compactness, along with the defining equations of any frobenius algebras or modules which appear is our equations, and of course given the state of knowledge $(f,\tau)$ we may use the equation which defines it.

%There are some statements $(f,\tau^{*})$ which can be derived from $(f,\tau)$ by just looking at the relations themselves, we call such deductions entailments.

\begin{definition}[Structural Equations]
$x = y$ is a structural equation in $\cat{V}$ if it follows from the defining equations of each frobenius algebra, cap, cup and module in $\cat{V}$.
\end{definition}
\begin{definition}[Structural Implication]
If statement $(f,\tau'): (A,Z) \rightarrow (B,W)$ is derivable from the statement $(f,\tau): (A,Z) \rightarrow (B,W)$ and structural equations, we say that $(f,\tau) > (f,\tau')$ and call the relation $``>"$ structural implication. 
\end{definition}
The relation
\begin{equation}
    (f,\tau) \sim (f,\tau') \iff (f,\tau) > (f, \tau')  \textbf{ and } (f,\tau') > (f, \tau) 
\end{equation}
is reflexive, transitive and the other one, as such it is an equivalence relation. We denote the equivalence classes as $[(f,\tau)]$. 
\subsubsection{Examples}
Using only structural deductions we can deduce $(\cap,\cap)$ from any $(\cap,\tau)$

\begin{equation}\label{samecapeq}
    \tikzfigscale{1}{cap}
\end{equation}


Considering a relation $\tau: X \rightarrow Y$ to be a subset of $X \times Y$, we inuitevely know that if $\tau' \subseteq \tau$ then $\tau'$ is a weaker statement than $\tau$. Formally this subset condition is presented in $\cat{V}$ by the following equation.
\begin{definition}[Subset]
$\tau$ is a subset of $\tau'$ written $\tau \subseteq \tau'$ if 
\begin{equation}\label{subset}
    \tikzfigscale{1}{subset}
\end{equation}

\end{definition}
\begin{theorem}[Subset Condition on Relations]
For all $\tau,\tau'$ such that $\tau \subseteq \tau'$: $(f,\tau) \implies (f\tau')$
\end{theorem}
\begin{proof}
\begin{equation}\label{subsetproof}
    \tikzfigscale{1}{subsetproof}
\end{equation}

\end{proof}
Put concisely, the natural partial order on relations lifts to a partial order on morphisms. 


Furthermore we can now use only structural deductions to show that $(\cap,\cap) > (\cap,\tau)$ for any $(\cap, \tau)$. We do this by showing that for any $(\cap,\tau)$ it must be the case that $\cap \subseteq \tau$. First of all note the following equations
\begin{equation}\label{provecup1}
    \tikzfigscale{1}{provecup1}
\end{equation}
Which in turn imply (we would need to include this bit, but its a fairly natural thing to ask for from the outset)
\begin{equation}\label{provecup2}
    \tikzfigscale{1}{provecup2}
\end{equation}
Then we can see that $\cap$ is a subset of $\tau$
\begin{equation}\label{provecup3}
    \tikzfigscale{1}{provecup3}
\end{equation}
and so it follows that $(\cap,\cap) > (\cap,\tau)$. We have found then that all morphisms of the form $(\cap,\tau)$ are equivalent by only structural deductions.


Furthermore in the equivalence class $[(f,\tau)]$ there is always a least member $\tau'$, the equivalence class is closed under taking intersections. 

\begin{definition}[Intersection]
The intersection of $\tau$ and $\tau'$ denoted $\tau \cap \tau'$ is given by 
\begin{equation}\label{intersection}
    \tikzfigscale{1}{intersection}
\end{equation}
\end{definition}
\begin{theorem}
$(f,\tau)$ and $(f,\tau')$ imply $(f,\tau \cap \tau')$.
\end{theorem}
\begin{proof}
\begin{equation}\label{intersectionproof}
    \tikzfigscale{1}{intersectionproof}
\end{equation}
\end{proof}



\subsubsection{The Problem!}
We have found a sense in which we should always be able to replace $(\cap,\tau)$ with $(\cap,\cap)$. The trouble comes when we try to say what we mean by such a replacement formally. One might anticipate the standard trick of taking the Quotient Category with respect to our equivalence relation: turning morphisms into equivalence classes. Sadly though, composition is not well defined for these equivalence classes. The following looks like a proof that they do, but there is a subtle mistake!
\begin{lemma}[Composition of Equivalence Classes]
\begin{equation*}
    (f,\tau) > (f, \tau') \wedge (g,\sigma) > (g, \sigma') \implies (f \circ g,\tau \circ \sigma) > (f \circ g, \tau' \circ \sigma')
\end{equation*}
\end{lemma}
\begin{proof}
\begin{equation*}
    (f \circ g,\tau \circ \sigma)  = (f, \tau) \circ (g,\sigma) = (f, \tau') \circ (g,\sigma') = (f \circ g,\tau' \circ \sigma')
\end{equation*}
\end{proof}
What went wrong? It's the first line, the statement 
\begin{equation*}
    (f \circ g,\tau \circ \sigma)  = (f, \tau) \circ (g,\sigma)
\end{equation*}
Does not actually follow from just the statement $(f \circ g,\tau \circ \sigma)$ and structural equations, since there is no garuntee that $\tau$ is a routing morphism for $f$. 

\subsubsection{Solutions}
\begin{itemize}
    \item Admit this is a dead end
    \item Ask why we ever wanted allowed replacements of routing maps to be compositional. Why not just replace any $(f,\tau)$ with any $(f,\tau')$ whenever we know that $(f,\tau')$ exists. Done, we have some morphism $(f,\tau)$, we can replace it with morphism $(f,\tau')$, we have the same $f$ as before and we have some new statement about it. What else is there to care about it.
    \item Hack a compositional version of the equivalence class. E.G Make some recursive definition like $(f,\tau) > (f,\tau')$ if $(f,\tau) = (f_1, \tau_1) \circ (f_2, \tau_2)$ and $(f,\tau') = (f_1, \tau_1') \circ (f_2, \tau_2')$ with $(f_1,\tau_1) > (f_1,\tau_1')$ and $(f_2,\tau_2) > (f_2,\tau_2')$.
\end{itemize}




